Efficient Semi-Supervised Learning for Natural Language Understanding by Optimizing Diversity

Expanding new functionalities efficiently is an ongoing challenge for single-turn task-oriented dialogue systems. In this work, we explore functionality-specific semi-supervised learning via self-training. We consider methods that augment training data automatically from unlabeled data sets in a functionality-targeted manner. In addition, we examine multiple techniques for efficient selection of augmented utterances to reduce training time and increase diversity. First, we consider paraphrase detection methods that attempt to find utterance variants of labeled training data with good coverage. Second, we explore sub-modular optimization based on n-grams features for utterance selection. Experiments show that functionality-specific self-training is very effective for improving system performance. In addition, methods optimizing diversity can reduce training data in many cases to 50% with little impact on performance.

==> related_work.tex <==
Popular SSL models include self-training, mixture models, graph-based methods, co-training and multiview learning ~\cite{zhu2005semi, zhu2009introduction, chapelle2010ssl}. Particularly, in speech and language processing, self-training~\cite{ma2006unsupervised,tur2005combining,mcclosky2006effective,reichart2007self} and methods that learn representations from implicit information are common~\cite{collobert2008unified,peters2018deep}. In \cite{oliver2018realistic}, authors shared their insights on how evaluation of SSL approaches should be made when using real-world settings. 

Diversity in SSL was considered for text categorization task \cite{li2013semi}. In this work, diversity is used to better exploit unlabeled data by using feature subspace classifiers. %As a comparison, we use diversity as a criterion to decrease the amount of training data necessary for maintaining the performance. 

The authors in \cite{wieting2015towards} investigated six models for paraphrase embedding, varying in terms of expressiveness and complexity including deep averaging network \cite{iyyer2015deep} and LSTM networks \cite{hochreiter1997long}. %Inspired by this work, we examined the six models for embedding and selected the best performing one for our experiments.
